CLUB: A Contrastive Log-ratio Upper Bound of Mutual Information

Mutual information (MI) minimization has gained considerable interests in various machine learning tasks. However, estimating and minimizing MI in high-dimensional spaces remains a challenging problem, especially when only samples, rather than distribution forms, are accessible. Previous works mainly focus on MI lower bound approximation, which is not applicable to MI minimization problems. In this paper, we propose a novel Contrastive Log-ratio Upper Bound (CLUB) of mutual information. We provide a theoretical analysis of the properties of CLUB and its variational approximation. Based on this upper bound, we introduce a MI minimization training scheme and further accelerate it with a negative sampling strategy. Simulation studies on Gaussian distributions show the reliable estimation ability of CLUB. Real-world MI minimization experiments, including domain adaptation and information bottleneck, demonstrate the effectiveness of the proposed method. The code is at https://github.com/Linear95/CLUB.

==> tables/DA_MNIST_bak.tex <==
\setlength{\tabcolsep}{2.4pt}
\begin{table}[t]\small
    \centering
    \begin{tabular}{l|cccc}
        \toprule
        \textbf{Method} & M$\rightarrow$MM & M$\rightarrow$U & U$\rightarrow$M & S$\rightarrow$M \\
        \midrule
        \textbf{Source-Only} & 59.9 & 76.7 & 63.4 & 67.1\\
        \midrule
        \multicolumn{5}{c}{MI-based Disentangling Frameworks} \\
        \midrule
        \textbf{NWJ} & 83.3 & 98.3 & 91.1 & 86.5 \\
        \textbf{MINE} & 88.4 & 98.1 & 94.8 & 83.4 \\
        \textbf{InfoNCE} & 85.5 & 98.3 & 92.7 & 84.1 \\
        \midrule
        \textbf{VUB} & 76.4 & 97.1 & 96.3 & 81.5\\
        \textbf{L1Out} & 76.2 & 96.3 & 93.9 & - \\
        \textbf{CLUB} & 93.7 & \textbf{98.9} & 97.7 & 89.7 \\
        \textbf{CLUB (Sample)} & \textbf{94.6} & \textbf{98.9} & \textbf{98.1} & \textbf{90.6} \\
        \midrule
        \multicolumn{5}{c}{Other Frameworks} \\
        \midrule
        \textbf{MMD}~\cite{long2015learning} & 76.9 & - & - & 71.1 \\
        \textbf{DANN}~\cite{ganin2016domain} & 81.5 & 77.1 & 73.0 & 71.1 \\
        \textbf{DSN}~\cite{bousmalis2016domain}  & 83.2 & 91.3 & - & 76.0 \\
        \textbf{MCD}~\cite{saito2017maximum} & 93.5 & 94.2 & 94.1 & \textbf{92.6} \\
        \bottomrule
    \end{tabular}
    \caption{ Performance of the proposed domain adaptation framework for MNIST (M), MNIST-M (MM), USPS (U), and SVHN (S). Different MI estimators are applied to the framework. Test classification accuracy is reported. Among MI-based disentangling framework, the top three methods are MI lower bounds, while the rest are MI upper bounds. Other methods are also compared with, including MMD, DANN, DSN, and MCD.}
    \label{tab:domain_adapt}
%    \vspace{-2mm}
\end{table}
